Automatic Machine Learning Derived from Scholarly Big Data

One of the challenging aspects of applying machine learning is the need to identify the algorithms that will perform best for a given dataset. This process can be difficult, time consuming and often requires a great deal of domain knowledge. We present Sommelier, an expert system for recommending the machine learning algorithms that should be applied on a previously unseen dataset. Sommelier is based on word embedding representations of the domain knowledge extracted from a large corpus of academic publications. When presented with a new dataset and its problem description, Sommelier leverages a recommendation model trained on the word embedding representation to provide a ranked list of the most relevant algorithms to be used on the dataset. We demonstrate Sommelier's effectiveness by conducting an extensive evaluation on 121 publicly available datasets and 53 classification algorithms. The top algorithms recommended for each dataset by Sommelier were able to achieve on average 97.7% of the optimal accuracy of all surveyed algorithms.

==> Abstract.tex <==
\begin{abstract}
	One of the challenging aspects of applying machine learning is the need to identify the algorithms %most suited 
	that will preform best for a given dataset and task. This process can be difficult, time consuming and requires a great deal of domain knowledge. We present \MethodName, an efficient fully-automated approach for algorithm recommendation. When presented with a new dataset, \MethodName explores the vast body of publicly-available academic work to identify relevant research that reports the application of machine learning to similar tasks. The framework then leverages collaborative filtering methods to propose a ranked list of relevant algorithms to be used on the dataset. We demonstrate the effectiveness of our approach by conducting an extensive evaluation on 120 datasets and 53 classification algorithms \gilad{we can use the term "relative maximal accuracy", but I'm not sure if we should}.
	
\end{abstract}
